Learning a Single Index Model from Anisotropic Data with vanilla Stochastic Gradient Descent

We investigate the problem of learning a Single Index Model (SIM)- a popular model for studying the ability of neural networks to learn features - from anisotropic Gaussian inputs by training a neuron using vanilla Stochastic Gradient Descent (SGD). While the isotropic case has been extensively studied, the anisotropic case has received less attention and the impact of the covariance matrix on the learning dynamics remains unclear. For instance, Mousavi-Hosseini et al. (2023b) proposed a spherical SGD that requires a separate estimation of the data covariance matrix, thereby oversimplifying the influence of covariance. In this study, we analyze the learning dynamics of vanilla SGD under the SIM with anisotropic input data, demonstrating that vanilla SGD automatically adapts to the data's covariance structure. Leveraging these results, we derive upper and lower bounds on the sample complexity using a notion of effective dimension that is determined by the structure of the covariance matrix instead of the input data dimension.

==> analysis.tex <==
\section{Proof Outline}
We will first analyze the population dynamic in Section \ref{sec:pop_dyn}, then control the effect of the noise in Section \ref{sec:emp_dyn}. A key step in the analysis is understanding how the weight $w^{(t)}$ evolves. We will show that their evolution is mainly driven by the signal direction $w^*$. Toward this end, it will be useful to decompose any vector $w\in \R^d$ as \[ w = \wsig +\wpe \] where $\wsig = \la w, w^* \ra w^*$ is the orthogonal projection of $w$ onto $w^*$ and $\wpe=w-\wsig$ is its orthogonal complement. 
%\paragraph{Additional notations.} Let us denote $\wsig=P_{w^*}(w)=\la w, w^* \ra w^*$ the orthogonal projection of $w$ on the subspace spanned by $w^*$ and let $\wpe=w-\wsig$ its orthogonal complement. Due to the anisotropy of the input, the scalar product induced by $Q$ defined for any $x, y \in \R^d$ by $\la x, y \ra_Q:=x^\top Qy$ will play an important role. In particular, a natural measure of the correlation between $w^{(t)}$ and $w^*$ is given by $m_t=\la \frac{w^{(t)}}{\norm{Q^{1/2}w^{(t)}}},\frac{w^*}{\norm{Q^{1/2}w^*}}\ra_Q $. 

\subsection{Analysis of the population dynamic}\label{sec:pop_dyn} In this section, we will focus on the population dynamic and assume that we have access to the population gradients $ \expec \nabla L$ instead of their empirical counterpart $\nabla L$. Contrary to the spherical SGD algorithm analyzed in the isotropic setting \citep{Arous2020OnlineSG}, the analysis of the vanilla SDG with anisotropic inputs is more involved for two reasons: \begin{itemize}
    \item Unlike the isotropic case, the natural geometry for our problem is the one induced by $Q$. However, the studied algorithm is agnostic of $Q$ and designed for Euclidean geometry.
    \item Since we don't add constraints on the weights, one needs to additionally control $\norm{w^{(t)}}$.
\end{itemize}  

\subsubsection{Evolution of $m_t$}\label{subsec:mt} Let's start by studying the evolution of the correlation $m_t$. By using the update rule for $w^{(t)}$ and projecting it onto $\frac{Qw^*}{\norm{Q^{1/2}w^*}}$ we obtain  \begin{align*}
    m_{t+1}&= \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t+1)}}}m_t- \frac{\eta}{\norm{Q^{1/2}w^{(t+1)}}} \expec_x y \sigma'(\la \frac{w^{(t)}}{\norm{Q^{1/2}w^{(t)}}}, x \ra) \la x, \frac{Qw^*}{\norm{Q^{1/2}w^*}}  \ra .
\end{align*}


 The results are summarized in the following lemma. See the Section in the appendix for formal proof.
 \begin{lemma}\label{lem:evol_mt} The sequence $(m_t)_{t}$ satisfies the following relation \[ m_{t+1} \geq  \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t+1)}}}m_t+ \eta \frac{ \norm{Q^{1/2}w^*}}{\norm{Q^{1/2}w^{(t+1)}}} c m_t^{k^*-1}.\]  
 \end{lemma}
%
In contrast to previous work, the evolution of the correlation $m_t$ is affected by the evolution of the weights $w^{(t)}$. For example, if $\norm{Q^{1/2}w^{(t+1)}}$ becomes too large, the information provided by the gradient could vanish. Also, if the evolution is too fast, the ratio $\frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t+1)}}}$ could be far away from $1$, preventing the sequence $m_t$ from escaping from a neighborhood of zero. \gb{control of this quantity should appear somewhere...}

In the next sub-sections, we will control the growth of weights and show that the aforementioned problems won't appear. Hence the dynamic of $m_t$ can be well approximated by \[ m_{t+1}\approx m_t+\tilde{\eta} m_t^{k^*-1}\] where $\tilde{\eta}$ is a learning rate proportional to $\eta$. Starting from $m_o$, Proposition 5.1 in \cite{Arous2020OnlineSG} shows that one needs $\frac{k^*-2}{\tilde{\eta} m_0^{k^*-2}}$ iterations to obtain a correlation $m_t$ of constant order. This result can also be derived heuristically by solving the associated differential equation $f'=\tilde{\eta} f^{k^*-1}$.

%In summary we have shown that \[ m_{t+1}\approx \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t+1)}}}m_t+ \frac{\eta \norm{Q^{1/2}w^*}}{\norm{Q^{1/2}w^{(t+1)}}} c m_t^{k^*-1}.\] Contrary to spherical SDG, where the weights are constraints, we need to control $\norm{Q^{1/2}w^{(t)}}$.  We are going to show that $\norm{Q^{1/2}w^{(t)}}$ remains approximately constant as long as $m_t< \delta < 1$. Using this result, the dynamic simplifies to \[ m_{t+1}\approx m_t+\eta \lambda cm_t^{k^*-1}.\] This is a similar relation to the one obtained in the isotropic setting \cite{Arous2020OnlineSG}.

\subsubsection{Evolution of the growth of $\norm{\wsig^{(t)}}$}

 First, let us study the evolution of the weight along the signal direction. Notice that \begin{align}
    \norm{\wsig^{(t+1)}} &= \norm{\wsig^{(t)}} -\eta \expec_x y\sigma'(\la w^{(t)}, x \ra )\la x, w^*  \ra \nonumber\\
    &= \norm{\wsig^{(t)}} - \norm{Q^{1/2}w^*}\eta \expec_xf^*(\la x, \frac{w^*}{\norm{Q^{1/2}w^*}}  \ra)\sigma'(\la \frac{w^{(t)}}{\norm{Q^{1/2}w^{(t)}}}, x \ra)\la x, \frac{w^*}{\norm{Q^{1/2}w^*}}  \ra \tag{by scaling invariance of $\sigma'$.}\nonumber\\
    &= \norm{\wsig^{(t)}} - \norm{Q^{1/2}w^*}\eta \expec_{z^*,z_t}z^*f^*(z^*)\sigma'(z_t)
\end{align}
where $z^*, z_t\sim \calN(0,1)$ are correlated normal r.v. such that $\expec(z^*z_t)=m_t$. By using the same decomposition techniques as in the previous section, one can show that as long as $m_t\leq \gamma $, we have $\expec_{z^*,z_t}z^*f(z^*)\sigma'(z_t) \approx -cm_t^{k^*-1}$ for some constant $c>0$ by Assumption \ref{ass:coeff}. As a consequence, the growth of $\norm{\wsig^{(t)}}$ is similar to the one of $m_t$.




\subsubsection{Initial conditions}
 As shown in Section \ref{subsec:mt}, the value of $m_0$ plays an important role in the dynamic and will determine the required sampled complexity. In the isotropic case, it is typically of order $d^{-1/2}$. We are now going to evaluate the typical correlation at initialization in the anisotropic setting. 
 
By Gaussian concentration inequalities, we have $|\la w^{(0)}, w^* \ra_Q| \approx \norm{Qw^*}$ and $\norm{Q^{1/2}w^{(0)}}^2\approx \Tr(Q)$. So we can assume that $m_0=\frac{\norm{Qw^*}}{\norm{Q^{1/2}w^*}\sqrt{\Tr(Q)}}$. If $Q=I_d$, we recover the condition $m_0=\frac{1}{\sqrt{d}}$. In general $\frac{\norm{Qw^*}}{\norm{Q^{1/2}w^*}\sqrt{\Tr(Q)}}$ is quite different from $\frac{1}{\sqrt{d}}$. For example, if the eigenvalues of $Q$ are close to zero except for a few of them, $\Tr(Q)$ can be of constant order. On the other hand, if $Qw^*$ is small, i.e., $Q$ is not well aligned with $w^*$, and there are not many samples in this direction, $m_0$ could be significantly smaller than $\frac {1}{\sqrt{d}}$. 

%Also observe that at initialization that $\norm{\wsig^{(0)}}\approx \frac{\theta}{\sqrt{d}}$ while $\norm{\wpe^{(0)}}\approx \theta$.

\subsubsection{Conclusion}

In analyzing the population dynamic, the learning rate $\eta$ plays no important role. However, choosing $\eta$ small enough to control the noise terms is essential, as it will become clearer in Section \ref{sec:emp_dyn}. With the choice of Theorem \ref{thm:main} $\eta = \norm{Q^{1/2}}^{-2}_F m_0^{1-k^*}$ we obtain a sample complexity of order $O(\norm{Q^{1/2}}_F\norm{Q^{1/2}w^*}^{-1} m_0^{2-2k^*})$. 
\gb{Make a comparison with \cite{anisoSIM}. Check the value of $\eta$, it is essential in the proof...}

%By using the same proof as in Proposition 5.1 in \cite{Arous2020OnlineSG}, we show that one needs $T\gtrsim \eta \lambda m_0^{-k^*+2}$ for $k^*\geq 2$. The sample complexity matches the one obtained by \cite{anisoSIM} under a spiked covariance matrix model. Interestingly, our algorithm doesn't require an estimate of the covariance matrix and is hence faster. Furthermore, our analysis works for general covariance matrices and gives insight into the dynamic of the vanilla SGD, while previous work considered more specialized algorithms. 

\subsection{Analysis of the empirical dynamic}\label{sec:emp_dyn}

Following \cite{Arous2020OnlineSG}, we can write $\nabla_{w^{(t)}} L = \expec (\nabla_{w^{(t)}} L) + H_t$ where $H_t$ is a centered martingale. 

\subsubsection{Decomposition of the dynamic}
Assume that $\norm{Q^{1/2}w^{(t)}}$ remains of order $\theta = 1$ as long as $t\leq T$. 
By using the previous signal plus noise decomposition and leveraging the result from Section \ref{sec:pop_dyn}, we obtain \begin{equation*}
    m_{t+1}\geq m_t + \tilde{\eta}m_{t-1}^{k^*-1}+ \left( \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t+1)}}} -1 \right)m_t + \frac{\eta}{\norm{Q^{1/2}w^*}}\la H_t, w^*\ra.
\end{equation*}

\gb{some terms should be analyzed in population dynamic!}

By unraveling the recursion, we get \begin{equation}
    m_{t+1}\geq m_0 + \tilde{\eta}\sum_{l=1}^{t}m_l^{k^*-1}+ \underbrace{\sum_{l=1}^{t} \left( \frac{\norm{Q^{1/2}w^{(l)}}}{\norm{Q^{1/2}w^{(l+1)}}} -1 \right)m_l}_{E_1} + \underbrace{\sum_{l=1}^{t}\frac{\eta}{\norm{Q^{1/2}w^*}}\la H_l, w^*\ra}_{E_2}.
\end{equation}

\subsubsection{Control of the directional martingal term of $E_2$}
\gb{Don't cite Arous too many times. Emphasize the differences !}
As in \cite{Arous2020OnlineSG}, one can use Doob maximal inequality to show that $|E_2| \lesssim \frac{\eta \sqrt{t}}{\norm{Q^{1/2}w^*}}$. By choice of $\eta$, this term is negligible compared to $m_T$.
\gb{add details}

\subsubsection{Control of the weights evolution} We need to show that $\norm{Q^{1/2}w^{(t)}}$ remains close to initialization during the training. Since $\norm{Q^{1/2}}=1$ by assumption, it is enough to control the evolution of $w^{(t)}$. Let us write $\Bar{w}^{(t)}$, the sequence of weights obtained from $m_0$ with population gradient updates. We have \[ w^{(t)}= \Bar{w}^{(t)}+ \eta \sum_{l=0}^t H_t.\]

We already know from Section \ref{sec:pop_dyn} that $\norm{\Bar{w}^{(t)}}\approx \norm{\Bar{w}^{(0)}}$ as long as $m_t\leq \gamma$. It remains to control the norm of the additional martingale term. Let $(u_i)$ a basis of eigenvector of $Q^{1/2}$ associated with eigenvalues $(\lambda_i)$. By using Doob's maximal inequality we obtain \[ \abs{\sum_{l=0}^t \la H_t, u_i \ra }\lesssim \lambda_i^2 \sqrt{t}.\] By consequence, for all $t\leq T$, we have \[ \norm{\eta \sum_{l=0}^t H_t} \leq \eta \norm{Q^{1/2}}_H\sqrt{t} \ll 1\] by choice of $\eta$. So, at each step, $\norm{w^{(t)}}\approx \norm{\Bar{w}^{(t)}}$.

\subsubsection{Control of $E_1$}

Recall that \[ Q^{1/2}w^{(t+1)}= Q^{1/2}w^{(t)}-\eta \expec y\sigma'(w^{(t)}, x)Q^{1/2}x + \eta Q^{1/2}H_t .\]
The analysis done in Section $\ref{sec:pop_dyn}$ shows that \[ \expec y\sigma'(w^{(t)}, x)Q^{1/2}x \approx c m_t^{k^*-1} \] so it remains to control the effect of the noise at each step. \gb{Actually it is a bit different, we have $Q$ instead of $Q^{1/2}$ and so we need to use a decomposition of $Qw^*$...}

Let us write $E_t= \eta Q^{1/2}H_t$ for simplicity. It is a centered r.v. such that $\expec E^2 \leq \eta^2 \norm{Q}^2_H$. We have \begin{align*}
    \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t+1)}}} -1&= \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t)}+ \eta \expec y\sigma'(w^{(t)}, x)Q^{1/2}x+E_t}} -1 \\
    &\leq \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t)}+E_t}-\eta m_t^{k^*-1}} -1\\
    &\leq \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t)}+E_t}}\left( 1+ \eta m_t^{k^*-1}\right) -1 \tag{by using the fact that $\norm{Q^{1/2}w^{(t)}}\approx 1$}.
\end{align*}


Similarly, we can bound \begin{align*}
    \frac{\norm{Q^{1/2}w^{(t)}}}{\norm{Q^{1/2}w^{(t)}+E}}-1 &= \frac{\norm{Q^{1/2}w^{(t)}}-\norm{Q^{1/2}w^{(t)}+E}}{\norm{Q^{1/2}w^{(t)}+E}}\\
    &= \frac{\norm{Q^{1/2}w^{(t)}}^2-\norm{Q^{1/2}w^{(t)}+E}^2}{\norm{Q^{1/2}w^{(t)}+E}(\norm{Q^{1/2}w^{(t)}}+\norm{Q^{1/2}w^{(t)}+E})}\\
    & =  \frac{-2\la Q^{1/2}w^{(t)}, E\ra -\norm{E}^2}{\norm{Q^{1/2}w^{(t)}+E}(\norm{Q^{1/2}w^{(t)}}+\norm{Q^{1/2}w^{(t)}+E})}.
\end{align*}
Since $\norm{E}\ll 1$ w.h.p. by choice of $\eta$, $\norm{Q^{1/2}w^{(t)}+E}\approx \norm{Q^{1/2}w^{(t)}}$ and by consequence the numerator is of order $2\norm{Q^{1/2}w^{(t)}}^2\approx 2$. Hence \[ \sum_l m_l \frac{\norm{E}^2}{\norm{Q^{1/2}w^{(l)}+E}(\norm{Q^{1/2}w^{(l)}}+\norm{Q^{1/2}w^{(l)}+E})}= o(\eta \sum_l cm_l^{k^*-1}).\]

It remains to show that w.h.p. \[ \sup_{u: \norm{u}\leq 1}\abs{\sum_t m_t\la u, E_t \ra} =o(1)\]
This can be done by using Doob's maximal inequality, the definition of $\eta$, and a union-bound argument.


\subsection{Strong recovery: the descent phase}
\gb{The previous analysis is valid as long as $m_t\leq 1$ ?}

==> framework_old.tex <==
\section{Statistical Framework}

\paragraph{Model.} We observe for $i=1 \ldots T$ i.i.d. samples $(x^{(i)},y^{(i)})\in \R^{d}\times [-1,1]$ generated by the following process: the inputs $x^{(i)}\sim \calN(0,Q)$ are generated from a Gaussian distribution with covariance matrix $Q$ and $y^{(i)}=f^*(\langle x^{(i)}, \frac{w^*}{\norm{Q^{1/2}w^*}} \rangle)$ where $w^*\in \calS^{d-1}$ and $f^*:\R\to [-1,1]$ is an unknown link function. The normalization factor $\norm{Q^{1/2}w^*}$ is introduced so that $\langle x^{(i)}, \frac{w^*}{\norm{Q^{1/2}w^*}}\rangle \sim \calN(0,1)$ and only affects the definition of $f^*$. W.l.o.g. we can assume that $\norm{Q}=1$.
%and $\norm{Q^{1/2}}_H\to \infty$ when $d\to \infty$.
We make further assumption of $f^*$.


 \begin{assumption} \label{ass:ie}We assume that the link function $f^*: \R \to [-1,1]$ is such that $\expec(f^*)=0$, $\expec (f^*)^2=1$ and  $f^*$ has information exponent $k^*$ defined as  \[ k^* = \min \lbrace k\geq 1 : \expec (f^* H_k) \neq 0 \rbrace\] where $H_k$ is the order $k$ Hermite polynomial (see Section \ref{app:hermite} for more details).     
 \end{assumption}
\begin{remark}
    We assumed for simplicity that $f^*$ takes value in $[-1,1]$. Still, we believe our analysis could be extended to the class of functions $f^*$ growing polynomially, i.e., there exists a constant $C>0$ and an integer $p$ such that for all $x\in \R$, $|f^*(x)|\leq C(1+|x|^p)$. For example, using Lemma 16 in \cite{anisoSIM}, one could obtain a uniform upper bound on $|y^{(i)}|$ and reduce to the case where $f^*(x)\in [-1,1]$ for all $x$.
\end{remark}



 

\paragraph{Estimation method.} Following the approach in \cite{Arous2020OnlineSG}, we employ the correlation loss function \[ L(y, \hat{y})= 1 -y\hat{y}.\]  Our method involves training a single neuron, defined as $f_w(x)=\sigma(w^\top x)$ with $w\in \R^d$ and $\sigma$ denotes the ReLU activation function, using vanilla gradient descent. The steps are as follows:
\begin{itemize}
    \item Sample $w'\sim \calN(0,I_d)$ and initialize $w^{(0)}=r \frac{w'}{\norm{w'}}$ where $r>0$ is a scaling parameter.
    \item Update the weight by SDG $w^{(t+1)}=w^{(t)}-\eta \nabla_{w^{(t)}}L(y^{(t)}, f_{w^{(t)}}(x^{(t)}))$ where $\eta>0$ is the learning rate.
\end{itemize}

%Previous work such as \cite{Arous2020OnlineSG, bietti2022learning, AbbeAM23} leverage spherical SDG to train the weights. This approach leads to direct control of the norm of the weights $w^{(t)}$ at each iteration, which is convenient for the analysis. Also, as a by-product, it gives an equivalent between minimizing a least square loss and the correlation loss. However, an important drawback of this approach occurs in the anisotropic setting: as shown in \cite{anisoSIM} the algorithm needs to be modified and incorporate some knowledge of the covariance matrix to succeed in the anisotropic setting. 

%\begin{remark} Unlike previous work such as \cite{Arous2020OnlineSG, bietti2022learning,anisoSIM}, which constrained the weights, our approach relies on vanilla gradient descent.This method offers two main advantages: computational efficiency, as it does not require the estimation of the covariance matrix $Q$ to compute $\norm{Q^{1/2}w^*}$ as in \cite{anisoSIM}, and simplicity, aligning more closely with common practices in neural network training.\end{remark}

Previous works such as \cite{Arous2020OnlineSG, bietti2022learning, AbbeAM23} leverage spherical SGD to control the norm of the weights $w^{(t)}$ at each iteration, simplifying theoretical analysis and establishing equivalences between minimizing the least squares loss and the correlation loss. However, in the anisotropic setting, this method has significant limitations. As shown by \cite{anisoSIM}, spherical SGD must be modified with knowledge of the covariance matrix $Q$ to succeed.

\begin{remark} In contrast, our approach uses vanilla gradient descent without constraining the weights. This provides two key advantages: (1) computational efficiency, as it eliminates the need to estimate the covariance matrix $Q$ and compute terms like $\norm{Q^{1/2}w^*}$, and (2) simplicity, aligning more closely with standard practices in neural network training. \end{remark}


==> infinite.tex <==
{\color{blue}Minh: I am using this color
\section{Hermite polynomials on Hilbert space}

{\bf White noise mapping}
%For the expression of the Radon-Nikodym density between two equivalent Gaussian measures on 
%$\Hcal$, 
%in the following
%we utilize the concept of {\it white noise mapping}, 
(see e.g. \cite{DaPrato:2006,DaPrato:PDEHilbert}).
%In the following, 
For $\mu = \Ncal(m, Q)$, $\ker(Q) = \{0\}$, we  define
%\begin{align}
$\Lcal^2(\Hcal, \mu) = \Lcal^2(\Hcal, \Bsc(\Hcal),\mu) = \Lcal^2(\Hcal, \Bsc(\Hcal), \Ncal(m,Q))$.
%\end{align}
Consider the following mapping
\begin{align}
	&W:Q^{1/2}(\Hcal) \subset \Hcal \mapto \Lcal^2(\Hcal,\mu), \;\; z  \in Q^{1/2}(\Hcal) \mapto W_z \in \Lcal^2(\Hcal, \mu),
	\\
	%\end{align}
	%defined by
	%\begin{align}
	&W_z(x) = \la x -m, Q^{-1/2}z\ra,  \;\;\; z \in Q^{1/2}(\Hcal), x \in \Hcal.
	%W_z(x) = \la x, Q^{-1/2}z\ra,
\end{align}
For any pair $z_1, z_2 \in Q^{1/2}(\Hcal)$, it follows from the definition of covariance operator
that $\la W_{z_1}, W_{z_2}\ra_{\Lcal^2(\Hcal,\mu)} = \la z_1, z_2\ra_{\Hcal}$ 
%\begin{align}
%	\la W_{z_1}, W_{z_2}\ra_{\Lcal^2(\Hcal,\mu)}
% \int_{\H}W_{z_1}(x)W_{z_2}(x)\Ncal(m,Q)(dx)
%\\
%&
%	&= \int_{\Hcal}\la x -m, Q^{-1/2}z_1\ra\la x-m, Q^{-1/2}z_2\ra\Ncal(m, Q)(dx)
%	\nonumber
%	\\
%	& = \la Q(Q^{-1/2}z_1), Q^{-1/2}z_2\ra 
%\nonumber
%\\
%&
%	= \la z_1, z_2\ra_{\Hcal}.
%\end{align}
so that the map $W:Q^{1/2}(\Hcal) \mapto \Lcal^2(\Hcal, \mu)$ is an isometry, that is
%\begin{align}
$||W_z||_{\Lcal^2(\Hcal,\mu)} = ||z||_{\Hcal}$, $z \in Q^{1/2}(\Hcal)$.
%\end{align}
Since $\ker(Q) = \{0\}$, the subspace $Q^{1/2}(\Hcal)$ is dense in $\Hcal$ and the map $W$ can be uniquely extended to all of $\Hcal$, as follows.
For any $z \in \Hcal$, let $\{z_n\}_{n\in \Nbb}$ be a sequence in $Q^{1/2}(\Hcal)$ with $\lim_{n \approach \infty}||z_n -z||_{\Hcal} = 0$.
Then $\{z_n\}_{n \in \Nbb}$ is a Cauchy sequence in $\Hcal$, so that by isometry, $\{W_{z_n}\}_{n\in \Nbb}$ is also
a Cauchy sequence in $\Lcal^2(\Hcal, \mu)$, thus converging to a unique element in $\Lcal^2(\Hcal, \mu)$.
Thus
%for any $z \in \H$, 
we can define
% the map
\begin{align}
	W: \Hcal \mapto \Lcal^2(\Hcal, \mu),  \;\;\; z \in \Hcal \mapto \Lcal^2(\Hcal, \mu)
\end{align}
by the following unique limit in $\Lcal^2(\Hcal, \mu)$
\begin{align}
	W_z(x) = \lim_{n \approach \infty}W_{z_n}(x) = \lim_{n \approach \infty}\la x-m, Q^{-1/2}z_n\ra.
\end{align}
The map $W: \Hcal \mapto \Lcal^2(\Hcal, \mu)$ is called the {\it white noise mapping}
associated with the measure $\mu = \Ncal(m,Q)$.


The following result is from Da Prato \cite{DaPrato:2006}(Lemma 9.5)
(Note: the constants in the Hermite polynomials are slightly different)

\begin{proposition} 
	\label{proposition:Hermite-Hilbert-orthogonality-white-noise-mapping}
	Let $\mu = \Ncal(0,Q)$ with $\ker(Q) = \{0\}$. Assume that $h,g \in \Hcal$ with $||h|| = ||g|| = 1$. Then
\begin{align}
\int_{\Hcal}H_n(W_h)H_m(W_g)d\mu = \delta_{n,m}[\la h, g\ra]^n.
\end{align}
\end{proposition}

\begin{corollary}
	\label{corollary:Hermite-orthogonality-Rd-nonisotropic}
	For $\Hcal = \R^d$,
	\begin{align}
		\bE_{x \sim \Ncal(0,Q)}[H_n(\la h, x\ra)H_m(\la g, x\ra)] = \delta_{n,m}[\la Qh, g\ra]^n.
	\end{align}
\end{corollary}
Note: This formula should also be valid for the case $\dim(\Hcal) = \infty$ (to be proved)
\begin{proof}
For $\Hcal = \R^d$ and $\mu = \Ncal(0,Q)$, the white noise mapping is $W_h(x) = \la Q^{-1/2}h, x\ra$. 
Proposition \ref{proposition:Hermite-Hilbert-orthogonality-white-noise-mapping} thus gives
\begin{align*}
	\int_{\R^d}H_n(\la Q^{-1/2}h, x\ra)H_m(\la Q^{-1/2}h, x\ra)d\Ncal(0,Q) = \delta_{n,m}[\la h, g\ra]^n
\end{align*}
Equivalently,
\begin{align*}
	\bE_{x \sim \Ncal(0,Q)}[H_n(\la Q^{-1/2}h, x\ra)H_m(\la Q^{-1/2}g, x\ra)] = \delta_{n,m}[\la h, g\ra]^n
\end{align*}
It thus follows that on $\R^d$,
\begin{align*}
	\bE_{x \sim \Ncal(0,Q)}[H_n(\la h, x\ra)H_m(\la g, x\ra)] = \delta_{n,m}[\la Q^{1/2}h, Q^{1/2}g\ra]^n = \delta_{n,m}[\la Qh, g\ra]^n.
\end{align*}
\end{proof}
}

==> intro_old.tex <==
\section{Introduction}
Single Index Models (SIM) are a class of high-dimensional functions $F:\R^d \to \R$ of the form \[ F(x)=f(\langle w^*, x\rangle)\] where $w^*\in \mathbb{S}^{d-1}$ is the relevant direction of the model and $f$ is a univariate function referred to as the \textit{link function}.  This expressive model encompasses, as a special case, the Generalized Linear Model where the link function is known and offers a way to address the curse of dimensionality. It can be extended to multiple directions, leading to the Multi-Index Model.

In recent years, SIM has become particularly popular in the theoretical deep learning literature, as it provides a simple framework to study the ability of neural networks to adapt to the latent low dimension of the problem. Unlike kernel methods, SIM offers insights into how neural networks can efficiently learn features and leverage underlying low-dimensional structures in high-dimensional data. In particular, when $f$ is a degree $p$ polynomial, it is known that kernel methods will require a sample complexity of order $O(d^p)$ to estimate a SIM, while a two-layer neural network will only require $O(d^{k^*})$ sample in the online setting where $k^*$ is the information exponent \citep{damian22a, Arous2020OnlineSG}.

Following the recent work of \cite{damian2024computationalstatistical}, it has been shown that one can go beyond the information exponent by reusing data in the training dynamic, as discussed in \cite{repetita24} and the references therein. The difficulty of estimating SIM with Stochastic Gradient Descent (SGD) is conjectured to be governed by the Generative exponent.

\subsection{Motivations}
While previous work focused primarily on the finite setting with isotropic covariates $x\sim \calN(0, I_d)$, there are only limited results for functional data. The recent work of \cite{functionalSIM24} proposes a Ridge regularized least square estimator to estimate the latent dimension $w^*$. However, their analysis is limited to link functions $f$ such that $\expec(f'(x^\top w^*))\neq 0$. This corresponds to the link function having an Information exponent equal to $1$. Without such an assumption, $\expec(YX)=0$, and the least square estimator is completely decorrelated from the signal $\beta^*$. This leads to the following question:

\begin{center}
    \textit{Can we adapt finite-dimension methods to the infinite-dimension setting? }
\end{center}


\subsection{Heuristic analysis in the finite dimension setting (with known link function)}
Here, we present a simple heuristic argument to explain how one can learn the direction $w^*$ with a sample complexity $O(d^{k^*-1})$. The exposition follows \cite{Smoothing23}. Assume that the link function $f$ is known and consider a class of estimator of the form $f(x^\top w)$ for $w\in \mathbb{S}^{d-1}$. Further assume that $f$ is normalized so that $\expec_x f^2(x)=1$. Consider the loss function $  L(w;x;y) := 1-f(x^\top w) y.$ The latent direction $w^*$ can be estimated by using algorithm \ref{alg:smoothed_sgd} where $\nabla_w$ denotes the spherical gradient with respect to $w$. That is, for a function $g: \R^d \rightarrow \mathbb{R}$, let $\nabla_w g(w) = (I - ww^\top)\nabla g(z) $ where $\nabla$ is the standard Euclidean gradient (evaluated at $w$).

\begin{algorithm}[h!]
\begin{flushleft}
    \textbf{Input:} learning rate schedule $\set{\eta_t}$, smoothing schedule $\set{\lambda_t}$, steps $T$. \end{flushleft}
        \begin{algorithmic}[1]
        \State Sample $w_0 \sim \texttt{Unif}(S^{d-1})$
        \For{$t \leq T$}
        \State Sample a fresh sample $(x_t,y_t)$. 
        \State $\hat w_{t+1} \leftarrow w_t - \eta_t \nabla_w L_{\lambda_t}(w_t;x_t;y_t)$.
        \State $w_{t+1} \leftarrow \hat w_{t+1}/\norm{\hat w_{t+1}}$.
        \EndFor
       \end{algorithmic}
\caption{Smoothed Online SGD}
\label{alg:smoothed_sgd}
\end{algorithm}

Let $\set{c_k}_{k \ge 0}$ be the Hermite coefficients of $f$, i.e.
    \begin{align*}
        f(x) = \sum_{k \ge 0} \frac{c_k}{k!} He_k(x) \text{ where } c_k = \expec_{x \sim N(0,1)}[f(x) He_k(x)].
    \end{align*}
The information exponent corresponds to the smallest $k^*$ such that $c_{k^*}\neq 0$. 

We define $\alpha_t := w_t \cdot w^*$ so that $\alpha_t \in [-1,1]$ measures our current progress. Furthermore, let $v_t := -\nabla L_{\lambda_t}(w_t;x_t;y_t)$. Recall that the online SGD update is:
\begin{align*}
    w_{t+1} = \frac{w_t + \eta_t v_t}{\norm{w_t + \eta_t v_t}} \implies \alpha_{t+1} = \frac{\alpha_t + \eta_t (v_t \cdot w^\star)}{\norm{w_t + \eta_t v_t}}.
\end{align*}
Using the fact that $v \perp w$ and $\frac{1}{\sqrt{1+x^2}} \approx 1-\frac{x^2}{2}$ we can Taylor expand the update for $\alpha_{t+1}$:
\begin{align*}
    \alpha_{t+1} = \frac{\alpha_t + \eta_t (v_t \cdot w^\star)}{\sqrt{1 + \eta_t^2 \norm{v_t}^2}} \approx \alpha_t + \eta_t (v_t \cdot w^\star) - \frac{\eta_t^2 \norm{v_t}^2 \alpha_t}{2} + O(\eta_t^3).
\end{align*}

This dynamic can be decomposed between a drift term and a martingale term. This latter can be handled by using the result of \cite{Arous2020OnlineSG}. So, we will focus on the former. 

Taking expectations with respect to the fresh batch $(x_t,y_t)$ gives:
\begin{align*}
    \expec[\alpha_{t+1}|\mathcal{F}_t] \approx \alpha_t + \eta_t \expec[v_t \cdot w^\star|\mathcal{F}_t] - \eta_t^2 \expec[\norm{v_t}^2|\mathcal{F}_t] \alpha_t/2
\end{align*}
so to guarantee a positive drift, we need to set $\eta_t \leq \frac{2\expec[v_t \cdot w^\star|\mathcal{F}_t]}{\expec[\norm{v_t}^2|\mathcal{F}_t] \alpha_t}$ which gives us the value of $\eta_t$  for $t \le T_1$. However, to simplify the proof sketch, we can assume knowledge of $\expec[v_t \cdot w^\star|\mathcal{F}_t]$ and $\expec[\norm{v_t}^2|\mathcal{F}_t]$ and optimize over $\eta_t$ to get a maximum drift of
\begin{align*}
    \expec[\alpha_{t+1}|w_t] \approx \alpha_t + \frac{1}{2\alpha_t} \cdot \underbrace{\frac{\expec[v_t \cdot w^\star|\mathcal{F}_t]^2}{\expec[\norm{v_t}^2|\mathcal{F}_t]}}_{\text{SNR}}.
\end{align*}

\paragraph{Evaluation of the SNR.}
The following property will play a key role in evaluating the SNR.

\begin{proposition}[Orthogonality Property]\label{prop:hermite_ortho}
Let $w,w^\star \in S^{d-1}$ and let $\alpha = w \cdot w^\star$. Then:
\begin{align*}
    \expec_{x \sim N(0,I_d)}[He_j(w \cdot x)He_k(w^\star \cdot x)] = \delta_{jk}k!\alpha^k.
\end{align*}
\end{proposition}
\begin{remark}
    It is unclear how this property can be extended to nonisotropic $x$. However, it is essential to obtain an analogous formula, perhaps with a different way of measuring the correlation. See also the work of \cite{anisoSIM} that considered Gaussian inputs with a spiked covariance matrix.  
    \Minh{See Corollary \ref{corollary:Hermite-orthogonality-Rd-nonisotropic} below}
\end{remark}

Letting $P_w^\perp := I - ww^T$ denote the projection onto the subspace orthogonal to $w$ we have:
\begin{align*}
    L(w) = \sum_{k \ge 0} \frac{c_k^2}{k!} [1-\alpha^k] \text{ and } \nabla L(w) = - (P_w^\perp w^\star)\sum_{k \ge 0} \frac{c_k^2}{(k-1)!} \alpha^{k-1}.
\end{align*}
As $\alpha \ll 1$ throughout most of the trajectory, the gradient is dominated by the first nonzero Hermite coefficient so up to constants: $\expec[v \cdot w^\star] = -\nabla L(w) \cdot w^\star \approx \alpha^{k^*-1}$. Similarly, a standard concentration argument shows that because $v$ is a random vector in $d$ dimensions where each coordinate is $O(1)$, $\expec[\norm{v}]^2 \approx d$. Therefore the SNR is equal to $\alpha^{2(k^*-1)}/d$ so with an optimal learning rate schedule,
\begin{align*}
    \expec[\alpha_{t+1}|\mathcal{F}_t] \approx \alpha_t + \alpha_t^{2k^*-3}/d.
\end{align*}
This can be approximated by the ODE $\alpha' = \alpha^{2k^*-3}/d$. Solving this ODE with the initial $\alpha_0 \asymp d^{-1/2}$ gives that the escape time is proportional to $d \alpha_0^{-2(k^*-1)} = d^{k^*-1}$. 

\begin{remark}
    A more complete analysis can be found in \cite{bietti2022learning}.
\end{remark}


\subsection{Related work}

\paragraph{Single Index Model with nonisotropic inputs.}
There are relatively few works that go beyond the isotropic setting. In the deep learning literature, the two most important works are the one of \cite{beyongG24} that considers a deterministic condition on the population gradient that is provably satisfied by some class of distribution (such as the uniform distribution on the sphere) and the already mentioned work of \cite{anisoSIM} that considered anisotropic Gaussian with a spike aligned with the signal $w^*$.

\paragraph{Single Index Model for Functional data.} The work of \cite{functionalSIM24} seems to be the main theoretical work under this statistical framework. Their result are limited to the case $k^*=1$.

==> main_results.tex <==
\section{Main Results}

Given the insight gained from the dynamic of the population gradient, we can state our main result. 

%\gb{The theorem is stated for $k^*\geq 3$ but can be extended to any $k^*$. Also there is a gap with \cite{Arous2020OnlineSG} where there are additional $\log d$ factors. Check carefully.}

 \begin{theorem}\label{thm:main} Assume that Assumptions \ref{ass:ie}, \ref{ass:coeff} and \ref{ass:init} hold and the initialization scaling $r$ is such that $\norm{Q^{1/2}w^{(0)}}=c_r\norm{Q^{1/2}w^*} $ for some constant $c_r\in (0,1]$.
 \begin{enumerate}[noitemsep, topsep=-\parskip, label=(\arabic*)]
     \item When $k^*\geq 3$, choose $\eta=\epsilon_d\frac{m_0^{k^*-2}\norm{Q^{1/2}w^*}^2}{\norm{Q^{1/2}}^2_F}$ where $\epsilon_d\underset{d\to \infty}{\to} 0$.
 %
 Then, after $T= \Omega( m_0^{2(2-k)}\frac{\norm{Q^{1/2}}^2}{\norm{Q^{1/2}w^*}^2})$ iterations, $w^{(T)}$ weakly recovers $w^*$, i.e. with probability $1-o(1)$, $m_T\geq \delta $ for some constant $\delta>0$.
 \item If $k^*=2$, the same result holds with the choices $\eta= \frac{\epsilon_d^{1.5}\norm{Q^{1/2}w^*}^2}{\norm{Q^{1/2}}^2_F}$ and $T= \frac{\norm{Q^{1/2}}^2_F}{\epsilon_d\norm{Q^{1/2}w^*}^2}$.
 \item  If $k^*=1$, the result holds with the choices $\eta= \frac{\epsilon_d^2\norm{Q^{1/2}w^*}^2}{\norm{Q^{1/2}}^2_F\log m_0}$ and $T= \frac{\norm{Q^{1/2}}^2_F}{\epsilon_d\norm{Q^{1/2}w^*}^2}$.
 \end{enumerate}
 If we further assume that Assumption \ref{ass:coeff} holds for $\gamma= 1$, then $w^{(T)}$ strongly recovers $w^*$, i.e. $m_T\geq 1-o(1)$ with probability $1-o(1)$.
 \end{theorem}

 \begin{remark}
     The typical order of magnitude of $m_0$ is $\upper$, as shown by concentration inequalities. See Section \ref{app:init} in the appendix. In particular, when $Q=I_d$, $m_0\approx \sqrt{d}^{-1}$ and our upper bounds matches the one obtained by \cite{Arous2020OnlineSG}. When the covariance matrix is aligned with $w^*$, one can have $\sqrt{d}\ll m_0$. This accelarates the convergence as shown experimentally in Section \ref{sec:xp}.
 \end{remark}

\begin{remark}Our bound is weaker than the one obtained by \cite{anisoSIM} that is of order $dm_0^{(2k^*-2)}$. However, their analysis in based on GF and hence cannot be implemented directly, whereas we analyzed a simple and popular algorithm used in practice. The discretization of the GF is not a straightforward task. As highlighted by our analysis, the choice of the learning rate is crucial and has an effect on the required sample complexity. We believe that this is main reason that explain why one can obtain better bound with GF. 
\end{remark}

\begin{remark} One could possible remove Assumption \ref{ass:coeff} and \ref{ass:init} by considering a two-layer neural. Since the assumption on initialization is satisfied with probability $1/2$, it will be satisfied by a constant proportion of them. Moreover, by training the second layer, we could approximate $f^*$, hence controlling the sign of the coefficient appearing in Assumption \ref{ass:coeff}. 
\end{remark}


 A common way to provide lower-bound on the required sample complexity for SGD like algorithm is to rely on the Correlated Statistical Query (CSQ) framework. It is described in Section \ref{app:csq}. 

 \begin{theorem}[CSQ lower-bound]\label{thm:csq} Assume that $\norm{Q^{1/2}}_F^2\gtrsim \norm{Q}_H\sqrt{\log d}$ and $\norm{Q}_F\gtrsim \sqrt{\log d}$. Let us denote \[ m = \frac{\norm{Q}_F}{\norm{Q^{1/2}}^2_F}.\] Then, for any integer $k\geq 1$, there exists a class $\calF_k$ of polynomial functions of degree $k$ such that any CSQ algorithm using a polynomial number of queries $q=O(d^C)$ requires a tolerance of order at most \[ \tau^2 \leq  e^{k/2}\] where $\epsilon = m\sqrt{\log (qm^{k/2})}$.
 \end{theorem}
 \begin{proof}
     The main difficulty is the construction of a large family of vectors having small correlations measured by the scalar product induced by $Q$. It is detailed in Section \ref{app:csq}. 
 \end{proof}
\begin{remark}
    By using the heuristic $\tau^2 = \frac{1}{\sqrt{n}}$ we obtain $n=\Omega(\log d^{k/2} d \left(\frac{\norm{Q}_F}{\norm{Q^{1/2}}^2_F}\right)^{k/2})$. The term $\frac{\norm{Q}_F}{\norm{Q^{1/2}}^2_F}$ corresponds to the average value of $m_0$ when $w^*\sim \calN(0, I_d)$. Similarly to previous work \citep{damian22a}, there is a gap in the dependence in $k$ between the upper-bound provided by Theorem \ref{thm:main} and the lower bound. \cite{Smoothing23} show this gap can be removed in the isotropic case by using a smoothing technique.  
\end{remark}
\begin{remark} Theorem \ref{thm:csq} doesn't cover the cases where $\norm{Q}_F\ll \sqrt{\log d}$ or $\norm{Q^{1/2}}_F^2\gtrsim \norm{Q}_F \sqrt{\log d}$, i.e. the cases where the eigenvalues of $Q$ are quickly decreasing. In these settings, estimating the matrix $Q$ and incorporating it into the algorithm could lead to qualitatively better bounds.     
\end{remark}
